Towards Digital Twins for the Description of Automotive Software Systems

We present models for automotive software that capture quantitative and qualitative aspects of software systems and the underlying hardware architecture. In particular, we consider different levels of computing power. These range from controllers up to the cloud. We present a modeling approach for software deployment taking different automotive requirements such as criticality, latency, memory, computational resources, and communication into account. Our models capture automotive software and hardware system configurations and can serve as digital twins that are digital counterparts of (usually) physical entities. Furthermore, we highlight connected research areas and challenges.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{A. Aldini and H. Wiklicky (Eds.): Quantitative Aspects\\
of Programming Languages and Systems 2019 (QAPL'19).\\
EPTCS 312, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.312.2}{10.4204/EPTCS.312.2}}
\pdfoutput=1

